Recursively Summarizing Books with Human Feedback

A major challenge for scaling machine learning is training models to perform tasks that are very difficult or time-consuming for humans to evaluate. We present progress on this problem on the task of abstractive summarization of entire fiction novels. Our method combines learning from human feedback with recursive task decomposition: we use models trained on smaller parts of the task to assist humans in giving feedback on the broader task. We collect a large volume of demonstrations and comparisons from human labelers, and fine-tune GPT-3 using behavioral cloning and reward modeling to do summarization recursively. At inference time, the model first summarizes small sections of the book and then recursively summarizes these summaries to produce a summary of the entire book. Our human labelers are able to supervise and evaluate the models quickly, despite not having read the entire books themselves. Our resulting model generates sensible summaries of entire books, even matching the quality of human-written summaries in a few cases ($\sim5\%$ of books). We achieve state-of-the-art results on the recent BookSum dataset for book-length summarization. A zero-shot question-answering model using these summaries achieves state-of-the-art results on the challenging NarrativeQA benchmark for answering questions about books and movie scripts. We release datasets of samples from our model.

==> Books summarization paper 2021 (arxiv-v2)/bertscore_length_table.tex <==
\begin{tabular}{ c  c c  c  c  c }
\toprule
& Length & BERTScore & Correlation & Slope & Adjusted BERTScore\\
\hline
175b full tree & 719 $\pm$ 321 & 0.182 $\pm$ 0.039 & -0.148 & -3.36e-6 & 0.174 \\ % opt5
175b first subtree & 806 $\pm$ 379  & 0.178 $\pm$ 0.048 & -0.080 & -1.78e-5 & 0.174 \\ 
6b full tree & 655 $\pm$ 308 & 0.125 $\pm$ 0.043 & -0.024 & -1.01e-5 & 0.123 \\
\bottomrule

\end{tabular} 




\begin{comment}
(RAW DATA DUMP

lengths 718.9347826086956 +- 321.49659557152876
scores 0.1820923273006211 +- 0.038653687598793326
corr -0.14806819301261015
slope -3.3631146934577576e-06 intercept 0.1267955458864916
at 1k 0.17708871750460972
at 1167.2k 0.1741121714714221
at 2k 0.15928640869367897
175bfirsttree
lengths 805.5652173913044 +- 378.65985953749146
scores 0.17779050216726636 +- 0.04784152173884577
corr -0.07982627154386489
slope -1.7802308810930752e-05 intercept 0.19489102631554048
at 1k 0.1758295115319844
at 1167.2k 0.17414319990697538
at 2k 0.16574391568862912
6b
lengths 654.5434782608696 +- 307.581074962128
scores 0.12459424109724553 +- 0.04306703537375656
corr -0.024019076856750806
slope -1.0085595843355276e-05 intercept 0.18591510737533967
at 1k 0.12343243119303385
at 1167.2k 0.12287011841628771
at 2k 0.1200693164995761

END RAW DATA DUMP)
\end{comment}

==> Books summarization paper 2021 (arxiv-v2)/booksum_table.tex <==
\begin{tabular}{ c  c c  c  c  c }
\toprule
& Abstractive & ROUGE-1 & ROUGE-2 & ROUGE-L & BERTScore \\
\hline
Extractive Oracle &  & \textbf{46.62} & 9.17 & \textbf{18.31} & 0.082 \\
\hline
BertExt &  & 36.71 & 6.16 & 13.40 & 0.028 \\
T5 zero-shot & \checkmark  & 35.43 & 5.62 & 12.02 & 0.011 \\
T5 fine-tuned & \checkmark & 39.46 & 7.69 & 13.77 & 0.060 \\
\hline
175b full tree RL & \checkmark & 41.51 & 10.46 & 16.88 & \textbf{0.1821} \\ % opt5
175b first subtree RL & \checkmark & 43.19 & \textbf{10.63} & 17.10 & 0.1778 \\ 
6b full tree RL & \checkmark & 36.79 & 7.22 & 14.84 & 0.1246 \\
\bottomrule
\end{tabular} 




\begin{comment}
(RAW DATA DUMP


175b
bertscore 0.1820923273006211
rouge1 0.4150825839572288
rouge2 0.1046498093822759
rougel 0.16878069658717965
175bfirsttree
bertscore 0.17779050216726636
rouge1 0.4319473499940995
rouge2 0.10634997022345498
rougel 0.1710136358487453
6b
bertscore 0.12459424109724553
rouge1 0.36785063062923734
rouge2 0.07229703389613733
rougel 0.14837402086510798

END RAW DATA DUMP)
\end{comment}

==> Books summarization paper 2021 (arxiv-v2)/narrativeqa_table.tex <==
\begin{tabular}{ c  c  c  c  c }
\toprule
& ROUGE-L & BLEU-1 & BLEU-4 & METEOR \\
\hline
BiDAF \citep{kovcisky2018narrativeqa} & 6.2 & 5.7 & 0.3 & 3.7 \\
BM25 + BERT \citep{mou2020frustratingly} & 15.5 & 14.5 & 1.4 & 5.0 \\
RoBERTa \citep{zemlyanskiy2021readtwice} & 18.0 & 18.0 & 2.6 & 5.4 \\
ETC \citep{zemlyanskiy2021readtwice} & 18.8 & 17.2 & 2.7 & 5.4 \\
ReadTwice \citep{zemlyanskiy2021readtwice} & 23.3 & 21.1 & 4.0 & 7.0 \\
Retriever + Reader \citep{izacard2020distilling} & 32.0 & 35.3 & 7.5 & 11.1 \\
\hline
175b full tree, depth 1 & 21.03 & 21.82 & 3.87 & 10.52 \\
\hline
\textbf{\textit{6b}} full tree, depth 1 & 17.01 & 19.09 & 2.75 & 8.53 \\
175b \textbf{\textit{first subtree}}, depth 1 & 21.55 & 22.27 & 4.24 & 10.58 \\
175b full tree, \textbf{\textit{depth 0}} & 18.47 & 20.29 & 3.16 & 9.04 \\


% 175b full tree, depth 1 & \textbf{27.89} & \textbf{26.93} & \textbf{6.84} & \textbf{12.56} \\ % opt5
% 175b full tree, depth 0 & 24.48 & 24.46 & 5.77 & 10.73 \\ % opt5
% 175b first subtree, depth 1 & 27.74 & 26.66 & 6.47 & 12.35 \\ 
% 175b first subtree, depth 0 & 24.83 & 24.63 & 5.85 & 10.89 \\
% 6b full tree, depth 1 & 24.45 & 24.37 & 5.64 & 10.80 \\
% 6b full tree, depth 0 & 21.29 & 22.34 & 5.01 & 9.36 \\
% 6b full tree, depth 1, 6B zero-shot & 12.66 & 14.82 & 1.71 & 6.10 \\
% 6b full tree, depth 0, 6B zero-shot & 11.90 & 14.26 & 1.74 & 5.49 \\
\bottomrule

\end{tabular} 



\begin{comment}
(RAW DATA DUMP


6b depth 0
all {'Bleu_1': 0.14264702153018685, 'Bleu_2': 0.0626243182144133, 'Bleu_3': 0.03163345181561652, 'Bleu_4': 0.01737342480379874, 'METEOR': 0.054882563469004025, 'ROUGE_L': 0.1189934901559137, 'CIDEr': 0.15599888773151738}
gutenberg {'Bleu_1': 0.14425833710577213, 'Bleu_2': 0.06524171279194715, 'Bleu_3': 0.03475395632766791, 'Bleu_4': 0.019618055703853467, 'METEOR': 0.05732222685254224, 'ROUGE_L': 0.12298512705305154, 'CIDEr': 0.16837421755886756}
movies {'Bleu_1': 0.1392099557673156, 'Bleu_2': 0.059099048482513176, 'Bleu_3': 0.027748817056198624, 'Bleu_4': 0.014637044356319495, 'METEOR': 0.05262982389474473, 'ROUGE_L': 0.1151085456094844, 'CIDEr': 0.1477144090110152}

6b depth 1
all {'Bleu_1': 0.14820921266233392, 'Bleu_2': 0.06513847072217269, 'Bleu_3': 0.03322342798722796, 'Bleu_4': 0.017147676876027175, 'METEOR': 0.0610165844252961, 'ROUGE_L': 0.12655514783053712, 'CIDEr': 0.17009260675876725}
gutenberg {'Bleu_1': 0.1549913729356591, 'Bleu_2': 0.06865502338480305, 'Bleu_3': 0.03468393462784513, 'Bleu_4': 0.017412942723984408, 'METEOR': 0.06334868571555421, 'ROUGE_L': 0.137563358202952, 'CIDEr': 0.18862411111063257}
movies {'Bleu_1': 0.13758567161859536, 'Bleu_2': 0.05985860128240337, 'Bleu_3': 0.030857586253739164, 'Bleu_4': 0.016437168362483417, 'METEOR': 0.05886647788684733, 'ROUGE_L': 0.11584117560452507, 'CIDEr': 0.15571280576630417}



175b opt 5 depth 0 (worse than opt4)
all {'Bleu_1': 0.24457504102939417, 'Bleu_2': 0.14444988361340397, 'Bleu_3': 0.09155563313699695, 'Bleu_4': 0.057684898788998774, 'METEOR': 0.1072592596717164, 'ROUGE_L': 0.24482414889329554, 'CIDEr': 0.5015406564918924}
gutenberg {'Bleu_1': 0.24579261978248185, 'Bleu_2': 0.1444588515393856, 'Bleu_3': 0.08903085787837843, 'Bleu_4': 0.05367938768784174, 'METEOR': 0.10665030272510312, 'ROUGE_L': 0.2391933044991684, 'CIDEr': 0.48678539200322885}
movies {'Bleu_1': 0.24338296102713144, 'Bleu_2': 0.14442189016864398, 'Bleu_3': 0.09388234499625185, 'Bleu_4': 0.061362590349392815, 'METEOR': 0.10781909867311468, 'ROUGE_L': 0.2503044866054862, 'CIDEr': 0.5203504093679845}


175b opt 5 depth 1 (better than opt4)
all {'Bleu_1': 0.26928707639788857, 'Bleu_2': 0.16454883573524132, 'Bleu_3': 0.1051367151119508, 'Bleu_4': 0.06841079820380365, 'METEOR': 0.1256391094341792, 'ROUGE_L': 0.27885053238672475, 'CIDEr': 0.6086204132051449}
gutenberg {'Bleu_1': 0.2692547261614728, 'Bleu_2': 0.1608683349823652, 'Bleu_3': 0.09934478200917927, 'Bleu_4': 0.06286108454365674, 'METEOR': 0.12293045075847403, 'ROUGE_L': 0.27064262795241273, 'CIDEr': 0.5744871227956347}
movies {'Bleu_1': 0.26917641197828746, 'Bleu_2': 0.16790350322121922, 'Bleu_3': 0.11049693581552661, 'Bleu_4': 0.07368955714055506, 'METEOR': 0.12814686979073164, 'ROUGE_L': 0.2868390479735402, 'CIDEr': 0.6455638663648143}

175b depth 0
all {'Bleu_1': 0.24626466266001515, 'Bleu_2': 0.14527299237262675, 'Bleu_3': 0.09192996866804465, 'Bleu_4': 0.05852952278864984, 'METEOR': 0.10892381914817202, 'ROUGE_L': 0.24829705349189193, 'CIDEr': 0.5108628627633636}
gutenberg {'Bleu_1': 0.2440953460337033, 'Bleu_2': 0.14216069438307916, 'Bleu_3': 0.08854045277398517, 'Bleu_4': 0.05533261554386207, 'METEOR': 0.10587643679467648, 'ROUGE_L': 0.24352182193310862, 'CIDEr': 0.48844973387931334}
movies {'Bleu_1': 0.24828298496733364, 'Bleu_2': 0.148199619122576, 'Bleu_3': 0.09516014349723088, 'Bleu_4': 0.061597926886011095, 'METEOR': 0.11176822396395868, 'ROUGE_L': 0.2529446480202255, 'CIDEr': 0.5360607637391342}

175b depth 1
all {'Bleu_1': 0.2665982910750706, 'Bleu_2': 0.16151793375189868, 'Bleu_3': 0.10197668364595713, 'Bleu_4': 0.06470598213027341, 'METEOR': 0.12348404635570304, 'ROUGE_L': 0.2773546744538817, 'CIDEr': 0.6152483249485189}
gutenberg {'Bleu_1': 0.26500396832981465, 'Bleu_2': 0.15862580065683388, 'Bleu_3': 0.09728412131460666, 'Bleu_4': 0.05973694458259943, 'METEOR': 0.12076916722335324, 'ROUGE_L': 0.2706989672910617, 'CIDEr': 0.5856256704526707}
movies {'Bleu_1': 0.2679830998187121, 'Bleu_2': 0.16421219731414166, 'Bleu_3': 0.1064201040834005, 'Bleu_4': 0.06945940193818147, 'METEOR': 0.1260193095440054, 'ROUGE_L': 0.2838324814065553, 'CIDEr': 0.6466623320246635}


175b_6b depth 0
all {'Bleu_1': 0.16377869825395772, 'Bleu_2': 0.07988942630413676, 'Bleu_3': 0.04402875757471244, 'Bleu_4': 0.02614336293881233, 'METEOR': 0.06644079088481715, 'ROUGE_L': 0.14734820900948226, 'CIDEr': 0.23754400910819412}
gutenberg {'Bleu_1': 0.1638411554945681, 'Bleu_2': 0.07998698496558, 'Bleu_3': 0.04274280931301401, 'Bleu_4': 0.02469873961906675, 'METEOR': 0.06547613878067562, 'ROUGE_L': 0.145519048034844, 'CIDEr': 0.22362805072225594}
movies {'Bleu_1': 0.16371017881259534, 'Bleu_2': 0.07979163968681814, 'Bleu_3': 0.04515727702894897, 'Bleu_4': 0.027423169079225956, 'METEOR': 0.06733809207598603, 'ROUGE_L': 0.14912847839171425, 'CIDEr': 0.254509776030912}

175b_6b depth 1
all {'Bleu_1': 0.16880486044206827, 'Bleu_2': 0.08333648247337602, 'Bleu_3': 0.04704641151170733, 'Bleu_4': 0.02795820954756408, 'METEOR': 0.07047728417678316, 'ROUGE_L': 0.1494279264803638, 'CIDEr': 0.24341853651398745}
gutenberg {'Bleu_1': 0.1721238706981998, 'Bleu_2': 0.08450743370516711, 'Bleu_3': 0.04652176730158373, 'Bleu_4': 0.02639702134591829, 'METEOR': 0.07093472290421521, 'ROUGE_L': 0.15228435579185293, 'CIDEr': 0.23490501504716038}
movies {'Bleu_1': 0.1624262534370885, 'Bleu_2': 0.08064007954200711, 'Bleu_3': 0.046662971239412265, 'Bleu_4': 0.028903482833706702, 'METEOR': 0.07004951252333635, 'ROUGE_L': 0.14664784658785465, 'CIDEr': 0.2557106339943823}


175bopt5_6b depth 0
all {'Bleu_1': 0.16017847131579438, 'Bleu_2': 0.07501213815499774, 'Bleu_3': 0.040216378678322014, 'Bleu_4': 0.02292411617100015, 'METEOR': 0.06301719192191803, 'ROUGE_L': 0.13825529569458508, 'CIDEr': 0.2093005676313767}
gutenberg {'Bleu_1': 0.161517505671679, 'Bleu_2': 0.07456318287732905, 'Bleu_3': 0.039068279059542424, 'Bleu_4': 0.021295042712906453, 'METEOR': 0.06477557952102245, 'ROUGE_L': 0.13976802735476565, 'CIDEr': 0.21725905701277395}
movies {'Bleu_1': 0.15887952970985836, 'Bleu_2': 0.07541729948947551, 'Bleu_3': 0.041266242343584024, 'Bleu_4': 0.024370585433854362, 'METEOR': 0.0613923593293056, 'ROUGE_L': 0.13678299779653638, 'CIDEr': 0.20490214949664007}



175bopt5_6b depth 1
all {'Bleu_1': 0.1694563921853094, 'Bleu_2': 0.0820200446631164, 'Bleu_3': 0.04612201398145752, 'Bleu_4': 0.02760945426346095, 'METEOR': 0.07053821959007033, 'ROUGE_L': 0.1503980804429037, 'CIDEr': 0.23614550296836836}
gutenberg {'Bleu_1': 0.17165149544862565, 'Bleu_2': 0.08268438322179794, 'Bleu_3': 0.04435893577601129, 'Bleu_4': 0.02414814345274897, 'METEOR': 0.07077226744617181, 'ROUGE_L': 0.15412539686981247, 'CIDEr': 0.2333166628244042}
movies {'Bleu_1': 0.16424810685894609, 'Bleu_2': 0.07988422777129794, 'Bleu_3': 0.046885207281938304, 'Bleu_4': 0.030095491836452833, 'METEOR': 0.07032483634662408, 'ROUGE_L': 0.14677039135226563, 'CIDEr': 0.2426094422504546}
 
 
6b_175b depth 0
all {'Bleu_1': 0.2233721459025606, 'Bleu_2': 0.1278999361791744, 'Bleu_3': 0.07974900287644736, 'Bleu_4': 0.05014231071883953, 'METEOR': 0.09364202877006239, 'ROUGE_L': 0.2129336791468073, 'CIDEr': 0.4176903902523798}
gutenberg {'Bleu_1': 0.22468401724118273, 'Bleu_2': 0.12638046361014316, 'Bleu_3': 0.07602739934432774, 'Bleu_4': 0.04664071239978749, 'METEOR': 0.09176617233501316, 'ROUGE_L': 0.20886099323681154, 'CIDEr': 0.3986377401718619}
movies {'Bleu_1': 0.22202438725201176, 'Bleu_2': 0.12927188527235264, 'Bleu_3': 0.08315604949274387, 'Bleu_4': 0.05343752886277483, 'METEOR': 0.09538728177531403, 'ROUGE_L': 0.2168975063493022, 'CIDEr': 0.4402928


6b_175b depth 1
all {'Bleu_1': 0.2437485809232449, 'Bleu_2': 0.1436705776383654, 'Bleu_3': 0.0888871652455678, 'Bleu_4': 0.05638144661785038, 'METEOR': 0.10795128466202704, 'ROUGE_L': 0.2445440691388785, 'CIDEr': 0.5103787886984945}
gutenberg {'Bleu_1': 0.24620572496662133, 'Bleu_2': 0.14427921981336417, 'Bleu_3': 0.08864641541031429, 'Bleu_4': 0.05727552301190067, 'METEOR': 0.10646877199526615, 'ROUGE_L': 0.23924542347390115, 'CIDEr': 0.49270138446110157}
movies {'Bleu_1': 0.2412043378850634, 'Bleu_2': 0.14300717297214938, 'Bleu_3': 0.08912362783663766, 'Bleu_4': 0.055386490096642656, 'METEOR': 0.10933226039261622, 'ROUGE_L': 0.24970108745243685, 'CIDEr': 0.5312428083776779}

empty_175b
all {'Bleu_1': 0.2539018179067534, 'Bleu_2': 0.14979318201059913, 'Bleu_3': 0.09620876729903632, 'Bleu_4': 0.06438616782477849, 'METEOR': 0.11636524074574124, 'ROUGE_L':
0.2296161220508473, 'CIDEr': 0.4416002176943096}
gutenberg {'Bleu_1': 0.23581551404676068, 'Bleu_2': 0.13298032703773985, 'Bleu_3': 0.0848212143833187, 'Bleu_4': 0.056308651717435966, 'METEOR': 0.10604194585909503, 'ROUGE_L': 0.20922166688439242, 'CIDEr': 0.36624193030022645}
movies {'Bleu_1': 0.2691769435947997, 'Bleu_2': 0.16488221792877103, 'Bleu_3': 0.10665131922334681, 'Bleu_4': 0.07192188011550102, 'METEOR': 0.1260914257595593, 'ROUGE_L': 0.24946545439696513, 'CIDEr': 0.5210054597776688}

empty_6b
all {'Bleu_1': 0.15753263536939466, 'Bleu_2': 0.07200100893038303, 'Bleu_3': 0.03828584033389237, 'Bleu_4': 0.021201478470286788, 'METEOR': 0.06056845665063302, 'ROUGE_L': 0.12246925085684764, 'CIDEr': 0.13818272962301642}
gutenberg {'Bleu_1': 0.15640294734576687, 'Bleu_2': 0.0717006997910435, 'Bleu_3': 0.03740390001551279, 'Bleu_4': 0.01909033766286841, 'METEOR': 0.060029943364601025, 'ROUGE_L': 0.12179612865931842, 'CIDEr': 0.13467632026123624}
movies {'Bleu_1': 0.1563640252980552, 'Bleu_2': 0.07126173380743542, 'Bleu_3': 0.0385633523289755, 'Bleu_4': 0.022632755281695463, 'METEOR': 0.06106656383253101, 'ROUGE_L': 0.12312438119003168, 'CIDEr': 0.14731770591378263}

wiki_175b
all {'Bleu_1': 0.5674012355906795, 'Bleu_2': 0.45473272519966607, 'Bleu_3': 0.3697859515956538, 'Bleu_4': 0.30119746595765867, 'METEOR': 0.34888613327465606, 'ROUGE_L': 0.5753479210534104, 'CIDEr': 1.78819198422983}
gutenberg {'Bleu_1': 0.5571876782658035, 'Bleu_2': 0.4420380211110028, 'Bleu_3': 0.3556297030613771, 'Bleu_4': 0.2860014603967752, 'METEOR': 0.3499692453595864, 'ROUGE_L': 0.57825800554839, 'CIDEr': 1.78244148027131}
movies {'Bleu_1': 0.5775305266135223, 'Bleu_2': 0.4673318931241275, 'Bleu_3': 0.38396552729649286, 'Bleu_4': 0.31656037332819165, 'METEOR': 0.3478793618239993, 'ROUGE_L': 0.5725156201253059, 'CIDEr': 1.7948413899979516}

wiki_6b
all {'Bleu_1': 0.28356243502367373, 'Bleu_2': 0.1952177619046789, 'Bleu_3': 0.1421418339727507, 'Bleu_4': 0.1059847587053478, 'METEOR': 0.17155859042251456, 'ROUGE_L': 0.2791381341867941, 'CIDEr': 0.6854714987825983}
gutenberg {'Bleu_1': 0.2854671280276683, 'Bleu_2': 0.195933615305367, 'Bleu_3': 0.1426904389441528, 'Bleu_4': 0.10727846533716962, 'METEOR': 0.17805935225811553, 'ROUGE_L': 0.28675610922652844, 'CIDEr': 0.7060966459223649}
movies {'Bleu_1': 0.28170236083838157, 'Bleu_2': 0.19451686350242725, 'Bleu_3': 0.14160282876419128, 'Bleu_4': 0.10467621651028121, 'METEOR': 0.1655040580632633, 'ROUGE_L': 0.2717237797883088, 'CIDEr': 0.6703600094528787}

END RAW DATA DUMP)
\end{comment}
